ReVar: Strengthening Policy Evaluation via Reduced Variance Sampling

This paper studies the problem of data collection for policy evaluation in Markov decision processes (MDPs). In policy evaluation, we are given a target policy and asked to estimate the expected cumulative reward it will obtain in an environment formalized as an MDP. We develop theory for optimal data collection within the class of tree-structured MDPs by first deriving an oracle data collection strategy that uses knowledge of the variance of the reward distributions. We then introduce the Reduced Variance Sampling (ReVar) algorithm that approximates the oracle strategy when the reward variances are unknown a priori and bound its sub-optimality compared to the oracle strategy. Finally, we empirically validate that ReVar leads to policy evaluation with mean squared error comparable to the oracle strategy and significantly lower than simply running the target policy.

==> algo.tex <==
\subsection{Confidence Bound Policy Evaluation (CB-PE)}

Let learner the execute $\pi^{k}_b$ in the underlying MDP to generate a single trajectory $\tau^{k}=\left\{s_{t'}^{k}, a_{t'}^{k}\right\}_{t'=0}^{H-1}$ with $a_{t'}=$ $\pi_{t'}^{k}\left(s_{t'}^{k}\right)$ and $s_{t'+1}^{k} \sim P_{t'}\left(\cdot \mid s_{t'}^{k}, a_{t'}^{k}\right) .$ 


Now we define a few notations. The beginning of an episode is denoted as $k$. We use the history information up to the end of episode $k-1$ (denoted as $\mathcal{H}_{<k}$ ) to form some statistics. We define:
\begin{align*}
&N_{t'}^{k}\left(s, a, s^{\prime}\right)=\sum_{i=0}^{k-1} 1\left\{\left(s_{t'}^{i}, a_{h}^{i}, s_{t'+1}^{i}\right)=\left(s, a, s^{\prime}\right)\right\} \\
&N_{t'}^{k}(s, a)=\sum_{i=0}^{k-1} 1\left\{\left(s_{t'}^{i}, a_{t'}^{i}\right)=(s, a)\right\}, \forall h, s, a
\end{align*}

This counts how many times $s, a, s^{\prime}$ and $s, a$ are visited at time step $t'$ from the beginning of the learning process to the end of the episode $k-1$. We use these statistics to form an empirical model:
$$
\widehat{P}_{t'}^{k}\left(s^{\prime} \mid s, a\right)=\frac{N_{t'}^{k}\left(s, a, s^{\prime}\right)}{N_{t'}^{k}(s, a)}, \forall t', s, a, s^{\prime}.
$$
We will now define the exploration bonus, denoted as $b_{t'}(s, a)$ for all $t', s, a$ as follows:
$$
b_{t'}^{k}(s, a)=2 H \sqrt{\frac{\ln (S A H K / \delta)}{N_{t'}^{k}(s, a)}}.
$$
Now we state the Confidence Bound Policy Evaluation below:
\begin{algorithm}
\caption{Confidence Bound Policy Evaluation (\cbpe)}
\begin{algorithmic}[1]
\State \textbf{Input:} Initialize $\pi^0_b$, $\D = \emptyset$
\State \textbf{Output:} $\wv^k$
\For{$k \in 0 \ldots K-1$}
\State Generate trajectory $\tau^k \leftarrow$ with $\pi^k_b$ of length $t$.
\State Let the history be $h^k = \{s_{t'},a_{t'},r_{t'},s'_{t'+1}\}_{t' \in \tau^k}$
\State $\D = \D \cup \{h^k\}$
\State $\wv^k = \mathrm{PE}(\pi_e, D)$
\State $\wP^k_t \leftarrow \mathrm{Build-Model}(\D)$
\State $r^k_t \leftarrow b^k_t$
\State $\pi_b^{k+1} \leftarrow \mathrm{Value-Iter}(\wP^k_t, r^k_t)$
\EndFor
\State \textbf{Return} $\wv^k$
\end{algorithmic}
\end{algorithm}




